Deep Learning for Cross-Technology Communication Design

Recently, it was shown that a communication system could be represented as a deep learning (DL) autoencoder. Inspired by this idea, we target the problem of OFDM-based wireless cross-technology communication (CTC) where both in-technology and CTC transmissions take place simultaneously. We propose DeepCTC, a DL-based autoencoder approach allowing us to exploit DL for joint optimization of transmitter and receivers for both in-technology as well as CTC communication in an end-to-end manner. Different from classical CTC designs, we can easily weight in-technology against CTC communication. Moreover, CTC broadcasts can be efficiently realized even in the presence of heterogeneous CTC receivers with diverse OFDM technologies. Our numerical analysis confirms the feasibility of DeepCTC as both in-technology and CTC messages can be decoded with sufficient low block error rate.

==> sections/ideas.tex <==
%!TEX root = ../main.tex

%%%
\section{Ideas}

The preamble pattern detection can be also performed by a NN as follows. We put the FFT samples to the ring buffer. The size of buffer is (F,T), where F is number of subcarriers, while T is length of preamble pattern in number of OFDM symbols. 
Every time a new row of samples is added to the buffer, NN tries to detec the learned preamble pattern. Probably, we have to have some measure how good was the detection to synchronize to the start of the frame.
Probably, NN will learn something similar like 2D cross-correlation. does it require less computation than CC?

